Resource Allocation in One-dimensional Distributed Service Networks with Applications

We consider assignment policies that allocate resources to users, where both resources and users are located on a one-dimensional line. First, we consider unidirectional assignment policies that allocate resources only to users located to their left. We propose the Move to Right (MTR) policy, which scans from left to right assigning nearest rightmost available resource to a user, and contrast it to the Unidirectional Gale-Shapley (UGS) matching policy. While both policies among all unidirectional policies, minimize the expected distance traveled by a request (request distance), MTR is fairer. Moreover, we show that when user and resource locations are modeled by statistical point processes, and resources are allowed to satisfy more than one user, the spatial system under unidirectional policies can be mapped into bulk service queueing systems, thus allowing the application of many queueing theory results that yield closed form expressions. As we consider a case where different resources can satisfy different numbers of users, we also generate new results for bulk service queues. We also consider bidirectional policies where there are no directional restrictions on resource allocation and develop an algorithm for computing the optimal assignment which is more efficient than known algorithms in the literature when there are more resources than users. Numerical evaluation of performance of unidirectional and bidirectional allocation schemes yields design guidelines beneficial for resource placement. \np{Finally, we present a heuristic algorithm, which leverages the optimal dynamic programming scheme for one-dimensional inputs to obtain approximate solutions to the optimal assignment problem for the two-dimensional scenario and empirically yields request distances within a constant factor of the optimal solution.

==> 00-abstract.tex <==
%%%!TEX PS-program = pdflatexmk
%%!TEX root = 1d_mascots19.tex
\begin{abstract}
We consider assignment policies that allocate resources to users, where both resources and users are located on a one-dimensional line $[0,\infty)$. First, we consider unidirectional assignment policies that allocate resources only to users located to their left.
%as exemplified here. Imagine a one-way city street with traffic flowing from right to left; a ride-sharing company has distributed its vehicles along the street, which are ready to pick up users waiting at various locations. Users equipped with smartphone ride-hailing apps can register their requests on a ride allocation system. The latter then attempts to service each user by assigning a vehicle with spare capacity located to the user's right such that the average ``pick up" distance is minimized. 
We propose the Move to Right ({\it MTR}) policy, which scans from left to right assigning nearest rightmost available resource to a user, and contrast it to the Unidirectional Gale-Shapley ({\it UGS}) matching policy. While both policies 
among all unidirectional policies, minimize the expected distance traveled by a request ({\it request distance}), {\it MTR} is fairer. 
%\dt{removed mention of fairer and variance.  Belongs in paper.}
Moreover, we show that when user and resource locations are modeled by statistical point processes, and resources are allowed to satisfy more than one user, the spatial system under unidirectional policies can be mapped into bulk service queueing systems,  thus allowing the application of many queueing theory results that yield closed form expressions. As we consider a case where different resources can satisfy different numbers of users, we also generate new results for bulk service queues.  We also consider bidirectional policies where there are no directional restrictions on resource allocation and develop an algorithm for computing the optimal assignment which is more efficient than known algorithms in the literature when there are more resources than users. Finally, numerical evaluation of performance of unidirectional and bidirectional allocation schemes yields design guidelines beneficial for resource placement.
%, e.g., assigning distributed analytics tasks to servers in vehicular sensor networks, and give an optimal policy that has lower time complexity than known algorithms in literature in resource rich regimes. Finally, numerical evaluation of performance of unidirectional and bidirectional allocation schemes yield design guidelines beneficial for resource placement.


%We consider the problem of analyzing unidirectional allocation policies for assigning requesters of various tasks to servers. We assume both requesters and servers are placed on a one dimensional line: $[0,\infty)$ with servers having finite capacities. We show the equivalence of two of the  unidirectional policies: Queue Matching and Move to Right ({\it MTR}) policy w.r.t ``expected distance traveled by a request'' ({\it request distance}). We start our analysis with the case when both requesters and servers are distributed according to two independent poisson processes. We map the spatial system to a temporal M/M/1 queue or a bulk service M/M/1 queue depending on the server capacity. Next we present results associated with the case when the servers are distributed according to a renewal process. We map the spatial unidirectional system to a temporal M/G/1 queue with the first customer having exceptional service time and derive expressions for exceptional service time under various inter-server distance distributions. We present numerical results to validate the claim. Next, we propose an optimal allocation policy in a bi-directional system and compare the performance of the unidirectional policies with that of optimal policy.
\end{abstract}
